On the surface chemisorption of oxidizing fine iron particles: insights gained from molecular dynamics simulations

Molecular dynamics (MD) simulations are performed to investigate the thermal and mass accommodation coefficients (TAC and MAC, respectively) for the combination of iron(-oxide) and air. The obtained values of TAC and MAC are then used in a point-particle Knudsen model to investigate the effect of chemisorption and the Knudsen transition regime on the combustion behavior of (fine) iron particles. The thermal accommodation for the interactions of $\mathrm{Fe}$ with $\mathrm{N_2}$ and $\mathrm{Fe_xO_y}$ with $\mathrm{O_2}$ is investigated for different surface temperatures, while the mass accommodation coefficient for iron(-oxide) with oxygen is investigated for different initial oxidation stages $Z_\mathrm{O}$, which represents the molar ratio of $\mathrm{O}/\left(\mathrm{O} + \mathrm{Fe}\right)$, and different surface temperatures. The MAC decreases fast from unity to 0.03 as $Z_\mathrm{O}$ increases from 0 to 0.5 and then diminishes as $Z_\mathrm{O}$ further increases to 0.57. By incorporating the MD-informed accommodation coefficients into the single iron particle combustion model,a new temperature evolution for single iron particles is observed compared to results obtained with previously developed continuum models. Specifically, results of the present simulations show that the oxidation process continues after the particle reaching the peak temperature, while previous models predicting that the maximum temperature was attained when the particle is oxidized to $Z_\mathrm{O} = 0.5$. Since the rate of oxidation slows down as the MAC decreases with an increasing oxidation stage, the rate of heat loss exceeds the rate of heat release upon reaching the maximum temperature, while the particle is not yet oxidized to $Z_\mathrm{O} = 0.5$. Finally, the effect of transition-regime heat and mass transfer on the combustion behavior of fine iron particles is investigated and discussed.

==> Appendices/Init_velocities.tex <==
\section{Incident velocities}\label{sec:incident_Vel}
The diatomic molecule is modelled as rigid rotaters, where the initial velocity of each atom is prescribed. Figure \ref{fig:RigidRotor} shows a schematic representation of the diatomic nitrogen molecule.
\begin{figure}[h]
    \centering
    {\includegraphics[width=0.5\columnwidth]{Figures/Appendix/RigidRotor.eps}}
    \caption{Schematic representation of the diatomic nitrogen molecule represented as a rigid rotor}%
     \label{fig:RigidRotor}
\end{figure}

The translational energies of the molecule are sampled from the flux-corrected Maxwell-Boltzmann (MB) distribution, where the three velocities are described via \citep{Mane2018}
\begin{equation} \label{eq:mb_vxy}
    f\left(v_{CoM,x,y}\right) = \left( \frac{\bar{m}}{2\pi k_\mathrm{B} T} \right)^{1/2} \exp{\left(\frac{- \bar{m} v_{CoM,x,y}^2}{2 k_\mathrm{B} T} \right)},
\end{equation}
\begin{equation} \label{eq:mb_vz}
    f\left(v_{CoM, z}\right) = \left( \frac{\bar{m}}{k_\mathrm{B} T} \right)^{1/2} v_{CoM,z} \exp{\left(\frac{- \bar{m} v_{CoM,z}^2}{2 k_\mathrm{B} T} \right)},
\end{equation}
where $f$ is the velocity distribution function, $\bar{m}$ the mass of the nitrogen molecule, $v$ the velocity, $k_\mathrm{B}$ the Boltzmann constant, and $T$ the temperature.

The rotational energy of the gas molecule was sampled according to the Boltzmann distribution \citep{Hazenberg2023}
\begin{equation} \label{eq:mb_rot}
    \frac{N_i}{N} = \frac{g_i}{Z_\mathrm{rot}} \exp \left(\frac{E_\mathrm{rot,i}}{k_\mathrm{B} T}\right),
\end{equation}
with $N$ is the population, $N_i$ the number of particles in a state, $g_i$ the degeneracy of the energy state i, $Z_\mathrm{rot}$ the partition function and $E_\mathrm{rot,i}$ the rotational energy of the state $i$. Since quantum effects cannot be handled in MD simulations, this distribution is assumed to be continuous.

For the nitrogen molecule, it holds that $m_1 = m_2 = m$ and we assume that that initially $x_1 - x_2 = R$, $y_1 - y_2 = 0$ and $z_1 - z_2 = 0$. The velocity vector of the atoms can be described as
\begin{equation}
    v_i = v_{CoM,i} \pm dv_i,
\end{equation}
with $v_{CoM,i}$ the center of mass velocity derived from Equations \ref{eq:mb_vxy} and \ref{eq:mb_vz} and $dv_i$ the velocity of the atom with respect to the center of mass. The latter term could be determined from the rotational energy.

For linear molecules, like nitrogen, there can be no rotational motion around the line of atoms. Therefore, the rotational energy can be written as
\begin{equation}
    E_\mathrm{rot} = \frac{L_y^2 + L_z^2}{2I},
\end{equation}
with $L_i$ the angular momentum and $I$ the inertia tensor. The inertia tensor for linear diatomic molecule can be written as
\begin{equation}
    I = \mu R^2,
\end{equation}
with $\mu = \frac{m^2}{\bar{m}}$ the reduced mass.

The angular momentum can be written as
\begin{equation}
    L = \bar{m} \left(dr \times dv \right),
\end{equation}
with $dr$ the distance of the atom wrt to the center of mass. For a three dimensional case, the angular momentum becomes
\begin{equation}
    L = \begin{pmatrix}
L_x \\
L_y \\
L_z \\
\end{pmatrix} = \bar{m} \begin{pmatrix}
dy dv_z - dz dv_y \\
dz dv_x - dx dv_z \\
dx dv_y - dy dv_x \\
\end{pmatrix}.
\end{equation}
Substituting $dy = dz = 0$ and $L_x = 0$, we find that \begin{equation}
    dv_y = - \frac{\sqrt{I E_{rot}}}{\bar{m} dx},
\end{equation}
\begin{equation}
    dv_z = \frac{\sqrt{I E_{rot}}}{\bar{m} dx},
\end{equation}
with $dx$ equal to $1/2R$.
